Federated Learning for Internet of Things: A Federated Learning Framework for On-device Anomaly Data Detection

Federated learning can be a promising solution for enabling IoT cybersecurity (i.e., anomaly detection in the IoT environment) while preserving data privacy and mitigating the high communication/storage overhead (e.g., high-frequency data from time-series sensors) of centralized over-the-cloud approaches. In this paper, to further push forward this direction with a comprehensive study in both algorithm and system design, we build FedIoT platform that contains FedDetect algorithm for on-device anomaly data detection and a system design for realistic evaluation of federated learning on IoT devices. Furthermore, the proposed FedDetect learning framework improves the performance by utilizing a local adaptive optimizer (e.g., Adam) and a cross-round learning rate scheduler. In a network of realistic IoT devices (Raspberry PI), we evaluate FedIoT platform and FedDetect algorithm in both model and system performance. Our results demonstrate the efficacy of federated learning in detecting a wider range of attack types occurred at multiple devices. The system efficiency analysis indicates that both end-to-end training time and memory cost are affordable and promising for resource-constrained IoT devices. The source code is publicly available at https://github.com/FedML-AI/FedIoT.

==> listing/BeLevel-SSFL.tex <==
\begin{algorithm}[h!]
\small
\SetKwInOut{Input}{input}\SetKwInOut{Output}{return}
\Input{$K, T, \lambda, \Theta^{(0)}, \{\theta_i^{(0)}\}_{k\in[K]}, s\text{: number of local iteration}, \beta\text{: learning rate}$}
\For{$t=0,\ldots,T-1$}{
    Server randomly selects a subset of devices $S^{(t)}$\\
    Server sends the current global model $\Theta^{(t)}$ to $S^{(t)}$\\
    \For{device $k \in S^{(t)}$ in parallel}{
        \begin{tikzpicture} [remember picture, overlay]
            \node at (3pt, 2pt) (a) {};
            \node at (352pt,-93pt) (b) {};
            \node[line width=0pt, rounded corners=2pt, fill=blue!18, fill opacity=0.3, rectangle, fit=(a) (b)] (x) {};
            \node[anchor=south east,inner sep=1pt] at (x.south east) {\scriptsize$\clientOpt$};
        \end{tikzpicture}%
        Sample mini-batch $B_k$ from local dataset $D_k$, and do $s$ local iterations\\
        \tcc{Optimize the global parameter $\Theta$ locally}listalgorithmname
        $Z_1, Z_2 \leftarrow f_{\Theta^{(t)}}(\Tau(B_k)), f_{\Theta^{(t)}}(\Tau(B_k))$\\
        $P_1, P_2 \leftarrow h_{\Theta^{(t)}}(Z_1), h_{\Theta^{(t)}}(Z_2)$\\
        $\Theta_k^{(t)} \leftarrow \Theta^{(t)} - \beta \nabla_{\Theta^{(t)}} \frac{\D(P_1, \widehat{Z_2}) + \D(P_2, \widehat{Z_1})}{2}$, where $\widehat{\cdot}$ stands for stop-gradient\\
        \tcc{Optimize the local parameter $\theta_k$}
        $z_1, z_2 \leftarrow f_{\theta_k}(\Tau(B_k)), f_{\theta_k}(\Tau(B_k))$\\
        $p_1, p_2 \leftarrow h_{\theta_k}(z_1), h_{\theta_k}(z_2)$\\
        $\theta_{k}\leftarrow\theta_{k}-\beta\nabla_{\theta_{k}}\left(\frac{\D(p1,\widehat{z_{2}})+\D(p2,\widehat{z_{1}})}{2}+\lambda\left\Vert \Theta^{(t)}-\theta_{k}\right\Vert _{2}^{2}\right)$\\
        Send $\Delta_k^{(t)}:=\Theta_k^{(t)}-\Theta^{(t)}$ back to server
    }
    \begin{tikzpicture} [remember picture, overlay]
        \node at (5pt, 5pt) (a) {};
        \node at (367pt, 0pt) (b) {};
        \node[line width=0pt, rounded corners=2pt, fill=green!18, fill opacity=0.3, rectangle, fit=(a) (b)] (x) {};
        \node[anchor=south east,inner sep=1pt] at (x.south east) {\scriptsize$\serverOpt$};
    \end{tikzpicture}%
    $\Theta^{(t+1)} \leftarrow \Theta^{(t)} + \sum_{k \in S^{(t)}} \frac{|D_k|}{|D|} \Delta_k^{(t)}$
}
\Output{$\{\theta_i\}_{i\in[n]}, \Theta^{(T)}$}
\caption{BiLevel-SSFL}
\label{alg:bilevel-ssfl}
\end{algorithm}


==> listing/FedAvg-LA.tex <==
\begin{algorithm}[h!]
\small
\SetKwInOut{Input}{input}\SetKwInOut{Output}{return}
\Input{$K, T, \lambda, \Theta^{(0)}, \{\theta_i^{(0)}\}_{k\in[K]}, s\text{: number of local iteration}, \beta\text{: learning rate}$}
\For{$t=0,\ldots,T-1$}{
    Server randomly selects a subset of devices $S^{(t)}$\\
    Server sends the current global model $\Theta^{(t)}$ to $S^{(t)}$\\
    \For{device $k \in S^{(t)}$ in parallel}{
        \begin{tikzpicture} [remember picture, overlay]
            \node at (3pt, 2pt) (a) {};
            \node at (352pt,-41.5pt) (b) {};
            \node[line width=0pt, rounded corners=2pt, fill=blue!18, fill opacity=0.3, rectangle, fit=(a) (b)] (x) {};
            \node[anchor=south east,inner sep=1pt] at (x.south east) {\scriptsize$\clientOpt$};
        \end{tikzpicture}%
        Sample mini-batch $B_k$ from local dataset $D_k$, and do $s$ local iterations\\
        \tcc{Optimize the global parameter $\Theta$ locally}
        $Z_1, Z_2 \leftarrow f_{\Theta^{(t)}}(\Tau(B_k)), f_{\Theta^{(t)}}(\Tau(B_k))$\\
        $P_1, P_2 \leftarrow h_{\Theta^{(t)}}(Z_1), h_{\Theta^{(t)}}(Z_2)$\\
        $\Theta_k^{(t)} \leftarrow \Theta^{(t)} - \beta \nabla_{\Theta^{(t)}} \frac{\D(P_1, \widehat{Z_2}) + \D(P_2, \widehat{Z_1})}{2}$, where $\widehat{\cdot}$ stands for stop-gradient\\
        Send $\Delta_k^{(t)}:=\Theta_k^{(t)}-\Theta^{(t)}$ back to server
    }
    \begin{tikzpicture} [remember picture, overlay]
        \node at (5pt, 5pt) (a) {};
        \node at (367pt, 0pt) (b) {};
        \node[line width=0pt, rounded corners=2pt, fill=green!18, fill opacity=0.3, rectangle, fit=(a) (b)] (x) {};
        \node[anchor=south east,inner sep=1pt] at (x.south east) {\scriptsize$\serverOpt$};
    \end{tikzpicture}%
    $\Theta^{(t+1)} \leftarrow \Theta^{(t)} + \sum_{k \in S^{(t)}} \frac{|D_k|}{|D|} \Delta_k^{(t)}$
}
\Output{$\{\theta_i\}_{i\in[n]}, \Theta^{(T)}$}
\caption{FedAvg-LA}
\label{alg:fedavg-la}
\end{algorithm}


==> listing/MAML-SSFL.tex <==
\begin{algorithm}[h!]
\small
\SetKwInOut{Input}{input}\SetKwInOut{Output}{return}
\Input{$K, T, \lambda, \Theta^{(0)}, \{\theta_i^{(0)}\}_{k\in[K]}, s\text{: number of local iteration}, \beta\text{: learning rate}, M$}
\For{$t=0,\ldots,T-1$}{
    Server randomly selects a subset of devices $S^{(t)}$\\
    Server sends the current global model $\Theta^{(t)}$ to $S^{(t)}$\\
    \For{device $k \in S^{(t)}$ in parallel}{
        \begin{tikzpicture} [remember picture, overlay]
            \node at (3pt, 2pt) (a) {};
            \node at (352pt,-126pt) (b) {};
            \node[line width=0pt, rounded corners=2pt, fill=blue!18, fill opacity=0.3, rectangle, fit=(a) (b)] (x) {};
            \node[anchor=south east,inner sep=1pt] at (x.south east) {\scriptsize$\clientOpt$};
        \end{tikzpicture}%
        Sample mini-batch $B_k, B_k^\prime$ from local dataset $D_k$, and do $s$ local iterations\\
        \tcc{Inner loop update}
        $\Theta_k^{\prime (t)} \leftarrow \Theta^{(t)}$\\
        \For{$m = 0, \ldots, M-1$}{
            $Z_1^\prime, Z_2^\prime \leftarrow f_{\Theta^{\prime (t)}}(\Tau(B_k^\prime)), f_{\Theta^{\prime (t)}}(\Tau(B_k^\prime))$\\
            $P_1^\prime, P_2^\prime \leftarrow h_{\Theta^{\prime (t)}}(Z_1^\prime), h_{\Theta^{\prime (t)}}(Z_2^\prime)$\\
            $\Theta_k^{\prime (t)} \leftarrow \Theta_k^{\prime (t)} - \beta \nabla_{\Theta_k^{\prime (t)}} \frac{\D(P_1^\prime, \widehat{Z_2^\prime}) + \D(P_2^\prime, \widehat{Z_1^\prime})}{2}$, where $\widehat{\cdot}$ stands for stop-gradient\\
        }
        \tcc{Outer loop update}
        $Z_1, Z_2 \leftarrow f_{\Theta^{\prime (t)}}(\Tau(B_k)), f_{\Theta^{\prime (t)}}(\Tau(B_k))$\\
        $P_1, P_2 \leftarrow h_{\Theta^{\prime (t)}}(Z_1), h_{\Theta^{\prime (t)}}(Z_2)$\\
        $\Theta_k^{(t)} \leftarrow \Theta^{(t)} - \beta \nabla_{\Theta^{(t)}} \frac{\D(P_1, \widehat{Z_2}) + \D(P_2, \widehat{Z_1})}{2}$\\
        Send $\Delta_k^{(t)}:=\Theta_k^{(t)}-\Theta^{(t)}$ back to server
    }
    \begin{tikzpicture} [remember picture, overlay]
        \node at (5pt, 5pt) (a) {};
        \node at (367pt, 0pt) (b) {};
        \node[line width=0pt, rounded corners=2pt, fill=green!18, fill opacity=0.3, rectangle, fit=(a) (b)] (x) {};
        \node[anchor=south east,inner sep=1pt] at (x.south east) {\scriptsize$\serverOpt$};
    \end{tikzpicture}%
    $\Theta^{(t+1)} \leftarrow \Theta^{(t)} + \sum_{k \in S^{(t)}} \frac{|D_k|}{|D|} \Delta_k^{(t)}$
}
\Output{$\{\theta_i\}_{i\in[n]}, \Theta^{(T)}$}
\caption{MAML-SSFL}
\label{alg:maml-ssfl}
\end{algorithm}

==> listing/PerFedSimSiam.tex <==
\begin{center}
\scalebox{0.85}{
\begin{minipage}{\linewidth}

\begin{algorithm}[H]
\small
\SetKwInOut{Input}{input}\SetKwInOut{Output}{return}
\Input{$K, T, \lambda, \Theta^{(0)}, \{\theta_i^{(0)}\}_{k\in[K]}, s\text{: number of local iteration}, \beta\text{: learning rate}$}
\For{$t=0,\ldots,T-1$}{
    Server randomly selects a subset of devices $S^{(t)}$\\
    Server sends the current global model $\Theta^{(t)}$ to $S^{(t)}$\\
    \For{device $k \in S^{(t)}$ in parallel}{
        \begin{tikzpicture} [remember picture, overlay]
            \node at (3pt, 2pt) (a) {};
            \node at (352pt,-87.5pt) (b) {};
            \node[line width=0pt, rounded corners=2pt, fill=blue!18, fill opacity=0.3, rectangle, fit=(a) (b)] (x) {};
            \node[anchor=south east,inner sep=1pt] at (x.south east) {\scriptsize$\clientOpt$};
        \end{tikzpicture}%
        Sample mini-batch $B_k$ from local dataset $D_k$, and do $s$ local iterations\\
        \tcc{Optimize the global parameter $\Theta$ locally}
        $Z_1, Z_2 \leftarrow f_{\Theta^{(t)}}(\Tau(B_k)), f_{\Theta^{(t)}}(\Tau(B_k))$\\
        $P_1, P_2 \leftarrow h_{\Theta^{(t)}}(Z_1), h_{\Theta^{(t)}}(Z_2)$\\
        $\Theta_k^{(t)} \leftarrow \Theta^{(t)} - \beta \nabla_{\Theta^{(t)}} \frac{\D(P_1, \widehat{Z_2}) + \D(P_2, \widehat{Z_1})}{2}$, where $\widehat{\cdot}$ stands for stop-gradient\\
        \tcc{Optimize the local parameter $\theta_k$}
        $z_1, z_2 \leftarrow f_{\theta_k}(\Tau(B_k)), f_{\theta_k}(\Tau(B_k))$\\
        $p_1, p_2 \leftarrow h_{\theta_k}(z_1), h_{\theta_k}(z_2)$\\
        $\theta_k \leftarrow \theta_k - \beta \nabla_{\theta_k}\left( \frac{\D(p1, \widehat{z_2}) + \D(p2, \widehat{z_1})}{2} 
            + \lambda \frac{\D(p1, P_1) + \D(p1, P_2) + \D(p2, P_1) + \D(p2, P_2)}{4} \right)$\\
        Send $\Delta_k^{(t)}:=\Theta_k^{(t)}-\Theta^{(t)}$ back to server
    }
    \begin{tikzpicture} [remember picture, overlay]
        \node at (5pt, 5pt) (a) {};
        \node at (367pt, 0pt) (b) {};
        \node[line width=0pt, rounded corners=2pt, fill=green!18, fill opacity=0.3, rectangle, fit=(a) (b)] (x) {};
        \node[anchor=south east,inner sep=1pt] at (x.south east) {\scriptsize$\serverOpt$};
    \end{tikzpicture}%
    $\Theta^{(t+1)} \leftarrow \Theta^{(t)} + \sum_{k \in S^{(t)}} \frac{|D_k|}{|D|} \Delta_k^{(t)}$
}
\Output{$\{\theta_i\}_{i\in[n]}, \Theta^{(T)}$}
\caption{Per-SSFL}
\label{alg:pfss}
\end{algorithm}

  
\end{minipage}%
}
\end{center}

